Heavy quarks at finite temperature

New incarnations of heavy-ion collision experiments are turning our attention to hard processes and a more fine-grained resolution of the QGP. In this endeavor quarkonia or open heavy flavors turn out to be versatile probes, which are usually described through models based on perturbative QCD, AdS, and effective field theories. The lattice provides nonperturbative input and constraints to such models.\newline In-medium bottomonia, the complex static quark-antiquark potential, and the heavy-quark momentum diffusion coefficient are key quantities where lattice gauge theory has recently achieved significant progress with impact for heavy-ion phenomenology. We review these lattice results, relate them to phenomenological applications, and close with an outlook.

==> macros.tex <==
% input and standard packages
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{lmodern}
\usepackage{default}
\usepackage{textcomp}
\usepackage{hyperref}

% %%%% graphics packages

\usepackage{blindtext}
\usepackage{graphicx}
% \usepackage{tcolorbox}
\usepackage{xcolor}
\usepackage{pgf}  
% \setlength{\unitlength}{10pt}
\newcommand{\ul}{\unitlength}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% input and standard packages
\usepackage{amsmath}
% \usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{fixmath}
\usepackage{braket}
\usepackage{slashed}
\usepackage{fontenc}
% \usepackage{dsfont}
\usepackage{bm}
\usepackage{xfrac}
\usepackage{mathtools}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tikz packages
\usepackage{tikz}
\usepackage[compat=1.1.0]{tikz-feynman}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{spy}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ist für Boxen (wie das hier benutzte Ovalbox) zuständig
\usepackage{fancybox}
\usepackage{adjustbox}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Einstellung des Eckenradius' der ovalen Boxen (\Ovalbox)
\cornersize*{5mm}
\linethickness{0.1mm}
\setlength{\fboxrule}{2.25mm}

%Ränder rechts/links
% \textwidth108mm
% \textheight1140mm
\textwidth144mm
\textheight216mm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% for Feynman diagrams
% \usepackage{feynmf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% colour definitions
\newcommand{\aka}{\color{red}}
% \newcommand{\ao}{\color{blue}}
\newcommand{\kuro}{\color{black}}
\newcommand{\shiro}{\color{white}}
\newcommand{\midori}{\color{ForestGreen}}
\newcommand{\DarkMagenta}{\color{DarkMagenta}}
\newcommand{\cha}{\color{brown}}

\definecolor{red}      {rgb}{0.8,0.0,0.0}
\definecolor{green}    {rgb}{0.0,0.6,0.0}
\definecolor{darkblue} {rgb}{0.0,0.1,0.7}
\definecolor{brown}    {rgb}{0.6,0.1,0.0}
\definecolor{gray}     {rgb}{0.6,0.6,0.6}
\definecolor{darkgreen}{rgb}{0.0, 0.545098, 0.0}
\definecolor{orange}   {RGB}{238,80,25}
\definecolor{purple}   {rgb}{0.5,0.0,0.5}
\definecolor{babypink} {rgb}{0.64, 0.44, 0.44}
\definecolor{bananayellow}{rgb}{1.0, 0.88, 0.21}

\definecolor{spartandarkgreen} {RGB}{24, 69, 59}
\definecolor{spartanlightgreen} {RGB}{13, 177, 75}
\definecolor{spartandarkgray} {RGB}{155, 162, 162}
\definecolor{spartanlightgray} {RGB}{153, 80, 84}

\definecolor{mytumgray}{HTML}{B0B0B0}
\definecolor{mytumblue}{HTML}{3071B5}
\definecolor{tumblue}{RGB}{0,101,189}
\definecolor{clustergray}{rgb}{0.459 , 0.502 , 0.569} %rgb 117,128,145 
\definecolor{clusterorange}{rgb}{1.0 , 0.620 , 0.145}%rgb 255,158,37

\definecolor{hu-berlin-blue}{RGB}{0,65,137} % HEX 004189
\definecolor{hu-berlin-green}{RGB}{150,190,20} % HEX 93C11A 
\definecolor{hu-berlin-grey}{RGB}{169,169,169}
\definecolor{hu-berlin-brown}{RGB}{82,79,60}
\definecolor{hu-berlin-red}{RGB}{180,0,0}
 
\newcommand{\sdgreen}{\color{spartandarkgreen}}
\newcommand{\slgreen}{\color{spartanlightgreen}}
\newcommand{\sdgray}{\color{spartandarkgray}}
\newcommand{\slgray}{\color{spartanlightgray}}
\newcommand{\tumgray}{\color{mytumgray}}
\newcommand{\tumblue}{\color{mytumblue}}
\newcommand{\white}{\color{white}}
\newcommand{\ucorange}{\color{clusterorange}}

\newcommand{\hublue}{\color{hu-berlin-blue}}
\newcommand{\hugreen}{\color{hu-berlin-green}}
\newcommand{\hugrey}{\color{hu-berlin-grey}}
\newcommand{\hubrown}{\color{hu-berlin-brown}}
\newcommand{\hured}{\color{hu-berlin-red}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% gluon decoration (based on the original coil decoration)

\pgfdeclaredecoration{gluon}{coil}
{
  \state{coil}[switch if less than=%
    0.5\pgfdecorationsegmentlength+%>
    \pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude+%
    \pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude to last,
               width=+\pgfdecorationsegmentlength]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{2    }{-0.555}{7}}
    {\pgfpoint@oncoil{1.555}{-1    }{8}}
    {\pgfpoint@oncoil{1    }{-1    }{9}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{0.445}{-1    }{10}}
    {\pgfpoint@oncoil{0    }{-0.555}{11}}
    {\pgfpoint@oncoil{0    }{ 0    }{12}}
  }
  \state{last}[next state=final]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
  }
  \state{final}{}
}

% \def\pgfpoint@oncoil#1#2#3{%
%   \pgf@x=#1\pgfdecorationsegmentamplitude%
%   \pgf@x=\pgfdecorationsegmentaspect\pgf@x%
%   \pgf@y=#2\pgfdecorationsegmentamplitude%
%   \pgf@xa=0.083333333333\pgfdecorationsegmentlength%
%   \advance\pgf@x by#3\pgf@xa%
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ellipse arc
\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % placeholder for possibly missing figures
% \let\StandardIncludeGraphics\includegraphics%
% \renewcommand{\includegraphics}[2][]{%
% \IfFileExists{#2.eps}{%
%   \StandardIncludeGraphics[#1]{#2}%
% }{%
%  \IfFileExists{#2.pdf}{%
%   \StandardIncludeGraphics[#1]{#2}%
%   }{ % No, no .pdf, try *.jpg 
%    \IfFileExists{#2.jpg}{%
%     \StandardIncludeGraphics[#1]{#2}%
%     }{
%       \IfFileExists{#2.png}{%
%       \StandardIncludeGraphics[#1]{#2}%
%       }{%
% %      \begin{tcolorbox}[width=6cm,height=4cm,arc=0mm,auto outer arc]
% %      \end{tcolorbox}
%      }
%    }
%  }
% }% 
% %
% }% End of command

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% highlightings
\newcommand{\dstyle}[1]{\footnotesize{$\ensuremath{\displaystyle{#1}}$}\small}
\newcommand{\tstyle}[1]{\tiny{$\ensuremath{\displaystyle{#1}}$}\small}
\newcommand{\squote}[1]{\texttt{\DarkMagenta \tiny [#1]}}
\newcommand{\stress}[1]{\textnormal{\aka #1}}
\newcommand{\highlight}[1]{\mathit{\aka #1}}
\newcommand{\name}[1]{\textsl{\ao #1}}
\newcommand{\trace}[1]{\ensuremath{\big\langle {#1}\big\rangle}}

 \newcommand{\circled}[2][6pt]{\raisebox{-#1}{\tikz{\node (F) at (0,0) {#2};\draw[thick](F)\circle(#1);}}}

\newcommand{\spartanitem}{\item[\color{spartandarkgreen}\(\bullet\)]}
\newcommand{\spartantitlebox}[1]{
 {\color{spartandarkgreen}\ovalbox{ \parbox{0.98\textwidth}{\color{spartandarkgreen}
  \center{\vskip-1ex\textbf{ #1}}
  \vskip.5ex
  }}}
}
\newcommand{\spartanbox}[1]{
 {\color{spartandarkgreen}\ovalbox{ \parbox{0.98\textwidth}{\color{spartandarkgreen}
  \vskip.5ex
  #1
  \vskip.5ex
  }}}
}
\newcommand{\smallspartanbox}[2]{
 {\color{spartandarkgreen}\ovalbox{ \parbox{#1\textwidth}{\color{spartandarkgreen}
  \vskip.5ex
  #2
  \vskip.5ex
  }}}
}
\newcommand{\tumbox}[1]{
 {\color{mytumblue}\ovalbox{ \parbox{0.98\textwidth}{\color{mytumblue}
  \vskip.5ex
  #1
  \vskip.5ex
  }}}
}
\newcommand{\smalltumbox}[2]{
 {\color{mytumblue}\ovalbox{ \parbox{#1\textwidth}{\color{mytumblue}
  \vskip.5ex
  #2
  \vskip.5ex
  }}}
}
\newcommand{\hubox}[1]{
 {\hublue\ovalbox{ \parbox{0.98\textwidth}{\hublue
  \vskip.5ex
  #1
  \vskip.5ex
  }}}
}
\newcommand{\smallhubox}[2]{
 {\hublue\ovalbox{ \parbox{#1\textwidth}{\hublue
  \vskip.5ex
  #2
  \vskip.5ex
  }}}
}

\newcommand{\prelimstamp}[1]{
{\rotatebox{#1}{\aka\ovalbox{\footnotesize\textbf{PRELIMINARY}}}}
}

%%%% mathematical formulas
\allowdisplaybreaks
\parindent 0pt
\parskip 10pt
% \numberwithin{equation}{section}
% \numberwithin{figure}{section}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% measure width of text
% \usepackage{calc}

\newenvironment{frcseries}{\fontfamily{frc}\selectfont}{}
\newcommand{\textfrc}[1]{{\frcseries#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% more generic macros for typesetting
\newcommand{\qgp}{quark-gluon-plasma}

%%%% macros for typesetting
\newcommand{\KW}{Karsten-Wilczek}
\newcommand{\BC}{Bori\c ci-Creutz}
\newcommand{\mido}{{minimally doubled}}
\newcommand{\mdf}{{\mido} fermion}
\newcommand{\mdfs}{{\mdf}s}
\newcommand{\Mdf}{Minimally doubled fermion}
\newcommand{\Mdfs}{{\Mdf}s}

%%%% macros for generic typesetting
\newcommand{\Eqref}[1]{\mbox{Eq.}~(\ref{#1})}
\newcommand{\Eqsref}[1]{\mbox{Eqs.}~(\ref{#1})}
\newcommand{\Figref}[1]{\mbox{Fig.}~\ref{#1}}
\newcommand{\ie}{\mbox{i.e.~}}
\newcommand{\eg}{\mbox{e.g.~}}

%%%% macros for fomulas
\renewcommand{\bm}{\mathbold}
\newcommand{\nn}{\nonumber}
\newcommand{\nnnl}{\nonumber\\}
\newcommand{\n}{\bm n}
\newcommand{\m}{\bm m}
\newcommand{\spr}{{^\prime}}
\newcommand{\adj}{{^\dagger}}
\newcommand{\inv}{{^{-1}}}
\newcommand{\vt}{\vartheta}
\newcommand{\ve}{\varepsilon}
\newcommand{\vepe}{\varepsilon^\perp}
\newcommand{\vepa}{\varepsilon^\parallel}
\newcommand{\lt}{\lambda}
\newcommand{\ups}{\upsilon}
\newcommand{\oh}[1]{\widehat{#1}}
\newcommand{\oha}[1]{\widehat{#1}\adj}
\newcommand{\sfs}{{\sf s}}
\newcommand{\sfx}{{\sf x}}
\newcommand{\sfy}{{\sf y}}
\newcommand{\sfz}{{\sf z}}
\newcommand{\sft}{{\sf t}}
\newcommand{\sftp}{{{\sf t}+1}}
\newcommand{\ksxyz}{{\kappa_{{\color{red}\sfs},{\color{purple}\sfx},{\color{darkblue}\sfy},{\color{darkgreen}\sfz}}}}
\newcommand{\ksyz}{{\kappa_{{\color{red}\sfs},{\color{darkblue}\sfy},{\color{darkgreen}\sfz}}}}
\newcommand{\kxyz}{{\kappa_{\sfx,\sfy,\sfz}}}
\newcommand{\ksy}{{\kappa_{\sfs,\sfy}}}
\newcommand{\ksz}{{\kappa_{\sfs,\sfz}}}
\newcommand{\kyz}{{\kappa_{\sfy,\sfz}}}
\newcommand{\kx}{{\kappa_{\sfx}}}
\newcommand{\ky}{{\kappa_{\sfy}}}
\newcommand{\kz}{{\kappa_{\sfz}}}
\newcommand{\ks}{{\kappa_{\sfs}}}
\newcommand{\gf}{{\gamma_5}}
\newcommand{\gt}{{\gamma_4}}
\newcommand{\gmu}[1]{{\gamma_{#1}}}
\newcommand{\gmup}[1]{{\gamma^\prime_{#1}}}
\newcommand{\gmunu}[2]{{\gamma_{#1}\gamma_{#2}}}
\newcommand{\smunu}[2]{{\Sigma_{#1#2}}}
\newcommand{\ptau}[1]{{P_\tau^{#1}}}
\newcommand{\pvt}[1]{{P_\vt^{#1}}}
\newcommand{\plt}[1]{{P_\lt^{#1}}}
\newcommand{\pf}[1]{{P_\chi^{#1}}}
\newcommand{\pc}[1]{{P_{\cal C}^{#1}}}
\newcommand{\pups}[1]{{P_\upsilon^{#1}}}

\newcommand{\abs}[1]{|#1|}
\newcommand{\arsinh}{\mathrm{arsinh}}
\newcommand{\arcosh}{\mathrm{arcosh}}
\newcommand{\artanh}{\mathrm{artanh}}
\newcommand{\as}{\alpha_s}
\newcommand{\als}{\as}
\newcommand{\Ntau}{{N_{\tau}}}
\newcommand{\Nsig}{{N_{\sigma}}}
\newcommand{\atau}{{a_{\tau}}}
\newcommand{\asig}{{a_{\sigma}}}
\newcommand{\lqcd}{\Lambda_{\textrm{\tiny QCD}}}
\def\lQ{\Lambda_{\rm QCD}}
\def\MS{\overline{\rm MS}}
\def\lMSbt{\Lambda_{\MS}^{N_f=3}}
\def\lMSb{\Lambda_{\MS}}
\newcommand{\aqq}{\alpha_{Q\bar Q}}
\newcommand{\Fqq}{F_{Q\bar Q}}
\newcommand{\fqq}{f_{Q\bar Q}}
\newcommand{\Fs}{F_S}
\newcommand{\fs}{f_S}
\newcommand{\Vs}{V_S}
\newcommand{\Fq}{F_Q}
\newcommand{\fq}{f_Q}
\newcommand{\qbq}{{Q\bar Q}}
\newcommand{\md}{m_D}
\newcommand{\tc}{T_c}
\newcommand{\nc}{N_c}
\newcommand{\nf}{N_f}
\newcommand{\cf}{C_F}
\newcommand{\ca}{C_A}
\renewcommand{\Re}[1]{{\rm Re}\,#1}
\renewcommand{\Im}[1]{{\rm Im}\,#1}
\newcommand{\sign}[1]{{\rm sign}\,(#1)\,}
% \newcommand{\ceil}[1]{{\left \lceil{#1}\right \rceil}}
\newcommand{\floor}[1]{{\left \lfloor{#1}\right \rfloor}}
\newcommand{\tr}[1]{{\rm Tr}\,#1}
\def\cdf{\chi^2/{\rm d.o.f.}}

%%%% macros from Stephan
\newcommand{\ri}{\mathrm{i}}
\newcommand{\si}{\sigma}
\newcommand{\ga}{\gamma}
\newcommand{\Si}{\Sigma}
\newcommand{\Ga}{\Gamma}

\newcommand{\rM}{\mathrm{M}}
\newcommand{\rD}{\mathrm{\Delta}}
\newcommand{\rT}{\mathrm{\Theta}}
\newcommand{\rP}{\mathrm{\Pi}}
\newcommand{\hS}{\hat{S}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\chS}{\mathcal{\hS}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bhS}{\bm{\hS}}

%%%% macros for colors
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\darkgreen}[1]{{\color{darkgreen}#1}}
\newcommand{\darkblue}[1]{{\color{darkblue}#1}}
\newcommand{\darkmagenta}[1]{{\color{purple}#1}}
\newcommand{\orange}[1]{{\color{orange}#1}}
\newcommand{\brown}[1]{{\color{brown}#1}}
\newcommand{\black}[1]{{\color{black}#1}}
\newcommand{\gray}[1]{{\color{Gray}#1}}

%%%% macros for generic math
\renewcommand{\bm}{\mathbold}
\newcommand{\mr}{\mathrm}
\newcommand{\mb}{\mathbf}
\newcommand{\mi}{\mathit}
\newcommand{\mf}{\mathfrak}
\newcommand{\mc}{\mathcal}
\def\ri{\mr{i}} 
\def\tr{\mr{tr}~}
\def\del{\partial} 
\def\nab{\nabla} 
\def\nabc{\nabla^{\ast}} 

%%%% macros for environments
\newcommand{\eq}[1]{\begin{equation}#1\end{equation}}
\newcommand{\al}[1]{\vskip-3ex\begin{align}#1\end{align}}
\newcommand{\eqlab}[1]{\begin{equation}#1\end{equation}}
\newcommand{\allab}[1]{\vskip-3ex\begin{align}#1\end{align}}
\newcommand{\alblank}[1]{\vskip-3ex\begin{align}#1\nonumber\end{align}}
\newcommand{\bmat}{\left(\begin{array}}
\newcommand{\emat}{\end{array}\right)}
\newcommand{\bvec}{\left(\begin{array}{c}}
\newcommand{\evec}{\end{array}\right)}
\newcommand{\quot}[1]{\begin{quote}#1\end{quote}}


\newcommand{\jhw}[1]{\textcolor{red}{\textbf{#1}}}

